Changing-look Active Galactic Nuclei from the Dark Energy Spectroscopic Instrument. I.Sample from the Early Data

Changing-look Active Galactic Nuclei (CL AGN) can be generally confirmed by the emergence (turn-on) or disappearance (turn-off) of broad emission lines, associated with a transient timescale (about $100\sim5000$ days) that is much shorter than predicted by traditional accretion disk models. We carry out a systematic CL AGN search by cross-matching the spectra coming from the Dark Energy Spectroscopic Instrument and the Sloan Digital Sky Survey. Following previous studies, we identify CL AGN based on $\rm{H}\alpha $, $\rm{H}\beta$, and Mg\,{\sc ii} at $z\leq0.75$ and Mg\,{\sc ii}, C\,{\sc iii}], and C\,{\sc iv} at $z>0.75$. We present 130 CL AGN based on visual inspection and three selection criteria, including 2 $\rm{H}\alpha$, 45 $\rm{H}\beta$, 38 Mg\,{\sc ii}, 61 C\,{\sc iii}], and 10 C\,{\sc iv} CL AGN. Twenty cases show simultaneous appearances/disappearances of two broad emission lines while three AGN exhibit the concurrent appearance of three broad emission lines. We also present 91 CL AGN candidates with significant flux variation of broad emission lines but remaining strong broad components. In the confirmed CL AGN, 42 cases show additional CL candidate features for different lines. In this paper, we find 1) a 95:35 ratio of a turn-on to turn-off CL AGN; 2) the highest redshift CL AGN ($z=3.56$) ever discovered; 3) an upper limit transition timescale ranging from 244 to 5762 days in the rest-frame; 4) the majority of CL AGN follow the bluer-when-brighter trend. Our results greatly increase the current CL census ($30\sim50\%$) and would be conducive to explore the underlying physical mechanism.

==> figure.tex <==


\begin{figure*}
% \addtocounter{figure}{-5}
\centering 
\includegraphics[width=0.47\textwidth]{075448.10+345828.5.pdf}\hspace*{0.01cm}
\includegraphics[width=0.47\textwidth]{085913.72+323050.8.pdf}\vspace*{0.01cm}
\includegraphics[width=0.47\textwidth]{095035.55+321601.0.pdf}\hspace*{0.01cm}
\includegraphics[width=0.47\textwidth]{103818.29+332437.2.pdf}\vspace*{0.01cm}
\includegraphics[width=0.47\textwidth]{113737.38+511839.9.pdf}\hspace*{0.01cm}
\includegraphics[width=0.47\textwidth]{115103.77+530140.6.pdf}\vspace*{0.01cm}
\includegraphics[width=0.47\textwidth]{115210.24+520205.1.pdf}\hspace*{0.01cm}
\includegraphics[width=0.47\textwidth]{115403.00+003154.0.pdf}\vspace*{0.01cm}
\includegraphics[width=0.47\textwidth]{121033.30-011755.6.pdf}\hspace*{0.01cm}
\includegraphics[width=0.47\textwidth]{122319.70+312737.0.pdf}\vspace*{0.01cm}
\caption{Appendix Figure for the rest of CL AGN.
}
\label{fig_example5}
\end{figure*}







\begin{figure*}
\addtocounter{figure}{-1}
\centering 
\includegraphics[width=0.47\textwidth]{125545.34+232348.0.pdf}\hspace*{0.01cm}
\includegraphics[width=0.47\textwidth]{125610.42+260103.4.pdf}\vspace*{0.01cm}
\includegraphics[width=0.47\textwidth]{133044.43+072628.8.pdf}\hspace*{0.01cm}
\includegraphics[width=0.47\textwidth]{133344.70+335622.7.pdf}\vspace*{0.01cm}
\includegraphics[width=0.47\textwidth]{134554.00+084537.3.pdf}\hspace*{0.01cm}
\includegraphics[width=0.47\textwidth]{135624.58+350813.1.pdf}\vspace*{0.01cm}
\includegraphics[width=0.47\textwidth]{135801.62+115331.8.pdf}\hspace*{0.01cm}
\includegraphics[width=0.47\textwidth]{140659.07+032601.9.pdf}\vspace*{0.01cm}
\includegraphics[width=0.47\textwidth]{140957.72-012850.5.pdf}\hspace*{0.01cm}
\includegraphics[width=0.47\textwidth]{141535.46+022338.7.pdf}\vspace*{0.01cm}
\caption{Continued.
}
\end{figure*}









\begin{figure*}
\addtocounter{figure}{-1}
\centering 
\includegraphics[width=0.47\textwidth]{141801.50+525200.7.pdf}\hspace*{0.01cm}
\includegraphics[width=0.47\textwidth]{141923.44-030458.7.pdf}\vspace*{0.01cm}
\includegraphics[width=0.47\textwidth]{144003.98+061936.5.pdf}\hspace*{0.01cm}
\includegraphics[width=0.47\textwidth]{144051.17+024415.8.pdf}\vspace*{0.01cm}
\includegraphics[width=0.47\textwidth]{145913.90+360051.4.pdf}\hspace*{0.01cm}
\includegraphics[width=0.47\textwidth]{152517.57+401357.6.pdf}\vspace*{0.01cm}
\includegraphics[width=0.47\textwidth]{152551.37+184552.0.pdf}\hspace*{0.01cm}
\includegraphics[width=0.47\textwidth]{152908.75+083203.5.pdf}\vspace*{0.01cm}
\includegraphics[width=0.47\textwidth]{153149.94+372755.4.pdf}\hspace*{0.01cm}
\includegraphics[width=0.47\textwidth]{153714.41+454347.7.pdf}\vspace*{0.01cm}
\caption{Continued.
}
\end{figure*}











\begin{figure*}
\addtocounter{figure}{-1}
\centering 
\includegraphics[width=0.47\textwidth]{153938.92+373853.8.pdf}\hspace*{0.01cm}
\includegraphics[width=0.47\textwidth]{154742.72+012541.0.pdf}\vspace*{0.01cm}
\includegraphics[width=0.47\textwidth]{160047.63+331310.7.pdf}\hspace*{0.01cm}
\includegraphics[width=0.47\textwidth]{160139.10+412529.3.pdf}\vspace*{0.01cm}
\includegraphics[width=0.47\textwidth]{160310.99+432928.9.pdf}\hspace*{0.01cm}
\includegraphics[width=0.47\textwidth]{160337.12+242513.9.pdf}\vspace*{0.01cm}
\includegraphics[width=0.47\textwidth]{160730.20+560305.5.pdf}\hspace*{0.01cm}
\includegraphics[width=0.47\textwidth]{161542.41+233143.9.pdf}\vspace*{0.01cm}
\includegraphics[width=0.47\textwidth]{161903.04+540529.0.pdf}\hspace*{0.01cm}
\includegraphics[width=0.47\textwidth]{162106.25+371950.7.pdf}\vspace*{0.01cm}
\caption{Continued.
}
\end{figure*}






\begin{figure*}
\addtocounter{figure}{-1}
\centering 
\includegraphics[width=0.47\textwidth]{164331.90+304835.5.pdf}\hspace*{0.01cm}
\includegraphics[width=0.47\textwidth]{164709.87+532202.2.pdf}\vspace*{0.01cm}
\includegraphics[width=0.47\textwidth]{164725.15+351754.3.pdf}\hspace*{0.01cm}
\includegraphics[width=0.47\textwidth]{164900.95+452016.8.pdf}\vspace*{0.01cm}
\includegraphics[width=0.47\textwidth]{213135.84+001517.0.pdf}\hspace*{0.01cm}
\includegraphics[width=0.47\textwidth]{213400.68+013828.4.pdf}\vspace*{0.01cm}
\includegraphics[width=0.47\textwidth]{213628.50-003811.8.pdf}\hspace*{0.01cm}
\includegraphics[width=0.47\textwidth]{221925.57+272806.4.pdf}\vspace*{0.01cm}
\includegraphics[width=0.47\textwidth]{223440.56+272437.9.pdf}\hspace*{0.01cm}
\includegraphics[width=0.47\textwidth]{224657.70-003242.5.pdf}\vspace*{0.01cm}
\caption{Continued.
}
\end{figure*}









